Minimalist exploration strategies for robot swarms at the edge of chaos

Effective exploration abilities are fundamental for robot swarms, especially when small, inexpensive robots are employed (e.g., micro- or nano-robots). Random walks are often the only viable choice if robots are too constrained regarding sensors and computation to implement state-of-the-art solutions. However, identifying the best random walk parameterisation may not be trivial. Additionally, variability among robots in terms of motion abilities-a very common condition when precise calibration is not possible-introduces the need for flexible solutions. This study explores how random walks that present chaotic or edge-of-chaos dynamics can be generated. We also evaluate their effectiveness for a simple exploration task performed by a swarm of simulated Kilobots. First, we show how Random Boolean Networks can be used as controllers for the Kilobots, achieving a significant performance improvement compared to the best parameterisation of a L\'evy-modulated Correlated Random Walk. Second, we demonstrate how chaotic dynamics are beneficial to maximise exploration effectiveness. Finally, we demonstrate how the exploration behavior produced by Boolean Networks can be optimized through an Evolutionary Robotics approach while maintaining the chaotic dynamics of the networks.

==> sections/2-related_works.tex <==
%\section{Background and Related Work}\label{RelatedWork}

% \begin{itemize}
%     \item \textcolor{red}{Alternatives for exploration tasks using autonomous agents (swarm or not?).}
%     \item \textcolor{red}{Works investigating/using/proposing random walk approaches.}
%     \item Works investigating chaotic dynamics for exploration.
%     \item Works within robotics field and RBN’s principles.
% \end{itemize}

%Swarm robotics (SR) is a research domain in exploration tasks that use autonomous agents without any centralized control or global knowledge. The global behavior of the swarm emerges from the local interactions of the robots. Swarm robotics systems usually present fault tolerance, flexible and scalable characteristics\cite{Sahin2005}. According to \cite{Brambilla2013}, there are two main design methods that can be used with robot swarms: (i) behaviour-based design and, (ii) automatic design. The first one often implies an iterative process to implement, analyse and improve the behavior of each robot until the desired collective behavior is obtained. It is the most common method for designing robot swarms and it is often inspired by well-know animal behaviours. The second is a method that allows the automatic design of the swarm behaviour without much intervention from the developer.

% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=3.2in]{figures/swarm_of_kilobots.png}
%     \caption{A swarm of Kilobots~\cite{kilobots}.}
%     \label{fig:SRKilobots}
% \end{figure}

%Random Walks are mathematical models of the movement presented by animals, cells and micro-organisms. For describing animal search patterns, the two more useful classes of RW are the correlated random walks (CRW) and the Lévy walks (LW)~\cite{Codling2008, Levy2015}. When using a behaviour-based design for a SR problem, these RWs are often adopted when the robots cannot rely on complex localization and mapping strategies, and therefore, cannot capitalize on environmental characteristics or social cues~\cite{Trianni2015}. Several studies utilizing RW are found in the literature. A biased CRW was implemented to solve a collective foraging task in~\cite{Hecker2015}. Random walks were utilized as mapping strategies in a close-space scenario in~\cite{Kegeleirs2019}. A CRW was utilized by robots in a collective decision-making problem in ~\cite{Reina2015}. In~\cite{Dimidov2016} the authors analyse the exploration efficiency of different sets of parameters for the LMCRW combined method. We used this last work as a reference of the best parameters for LMCRW, since the tasks and the robots used are the same in both works.

%Dynamical systems are capable of presenting three different dynamics: \textit{ordered, critical} and \textit{chaotic}. \textit{Chaotic} dynamics are characterized by an aperiodic bounded behaviour that is extremely sensitive to initial conditions~\cite{kaplan1997}. An \textit{ordered} regime, on the other hand, does not have sensitivity in the initial conditions so it always tends to the same attractor. \textit{Critical} dynamics are found ``at the edge'' between order and chaos. This dynamic can propagate small changes in the system when they are ``perturbed'' but at the same time preserve information~\cite{CarlosRBN}, which means that the changes are not completely random. As Langton proposed in~\cite{LANGTON1990}, living systems can find optimal conditions for life when they are in a regime close to the edge of chaos, since they get the required stability to survive and at the same time can freely explore new possibilities. 
%In \cite{DaRold2015}, the robot's controllers that evolved strategies producing chaotic dynamics lead to better performance both for environments previously experienced and in new environments. The authors have also demonstrated that the level of chaos (high sensitivity on initial conditions) is important too due to the fact the best results are obtained by the robots which have evolved a strange attractor with a lower dimension, suggesting a quasi-optimal level of chaos. In \cite{VOLOS2013} a microcontroller implementing a Chaotic Random Bit Generator based on a Logistic Map had success for controlling an autonomous mobile robot to cover an workspace within the fastest time possible.

The Genetic Regulatory Network (GRN) is a model that describes the interactions and dynamics between genes. A particular GRN is the Random Boolean Network (RBN), introduced by Kauffman~\cite{KAUFFMAN1969} as an abstract model of gene regulatory networks. In the robotics field, thanks to their compactness and readability, RBNs are used as robot programs capable of performing tasks such as \textit{phototaxis}, obstacle avoidance, and even synthesize finite state machines (FSM)~\cite{Roli2011,Garattoni2013,Roli2013}. In these works, the RBNs are synthesized through an automatically design methodology that uses meta-heuristic algorithms to modify its structure in order to fulfill its task.

A Random Boolean Network is a network with $N$ nodes representing genes with a boolean state indicating if the gene is expressed or not and is linked to the other nodes through $K$ directed edges. An edge from one node to the other implies that the former gene regulates the latter—$0$ and $1$ values on the edge indicate the presence/absence of activating/repressing proteins. The RBN is a discrete-state and discrete-time \textit{autonomous} system, which means that it evolves through time without any external inputs, despite, of course, its initial state \cite{Shmulevich2009}. The network activation is synchronous: the states of nodes at time $t+1$ depend on the states of nodes at time $t$. Usually, an initial random state is generated for the RBN, and the dynamics flow according to a set of predefined rules. These rules are randomly generated logic functions ($f$), assigned for each node, that use the input connections to define a new Boolean value. By using these rules, we can calculate all possible transient states of the given network. Since the state space is finite ($2^N$), eventually a state will be repeated~\cite{CarlosRBN}. 

Many variations of the RBN models have been proposed over time, so in this study, we will focus on the non-homogeneous RBNs introduced by Derrida and Pomeau~\cite{Derrida1986}. Different from the classical model proposed by Kauffman, the $K$ connections in this model are not the same for every node, so for e.g. we can have a node with $K=5$ and another with $K=0$. Removing this constraint allows us to explore a vast number of different networks and dynamics.

Despite many works investigating swarm robotics, exploration behavior with random walks, RBNs, and their application to robotics, just a few works propose the combination of random walks and critical or chaotic dynamics. Our work proposes an investigation in that direction.







